Algorithmic Recourse: from Counterfactual Explanations to Interventions

As machine learning is increasingly used to inform consequential decision-making (e.g., pre-trial bail and loan approval), it becomes important to explain how the system arrived at its decision, and also suggest actions to achieve a favorable decision. Counterfactual explanations -- "how the world would have (had) to be different for a desirable outcome to occur" -- aim to satisfy these criteria. Existing works have primarily focused on designing algorithms to obtain counterfactual explanations for a wide range of settings. However, one of the main objectives of "explanations as a means to help a data-subject act rather than merely understand" has been overlooked. In layman's terms, counterfactual explanations inform an individual where they need to get to, but not how to get there. In this work, we rely on causal reasoning to caution against the use of counterfactual explanations as a recommendable set of actions for recourse. Instead, we propose a shift of paradigm from recourse via nearest counterfactual explanations to recourse through minimal interventions, moving the focus from explanations to recommendations. Finally, we provide the reader with an extensive discussion on how to realistically achieve recourse beyond structural interventions.

==> 070broader_impact.tex <==
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss 

% a) who may benefit from this research, 

% b) who may be put at disadvantage from this research, 

% c) what are the consequences of failure of the system, and 

% d) whether the task/method leverages biases in the data.

% If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

Our work falls in the area of explainable AI, and focuses on the interpretability of algorithmic decision-making systems in consequential contexts, such as risk assessment, loan approval, hiring processes, among others. In particular, we address the fundamental limitations of using nearest counterfactual explanations to provide individuals with recourse actions. We do so by relying on causal reasoning, where actions correspond to interventions that do not only account for changes in the intervened variables, but also for downstream effects of such interventions on other variables, and thus, in the outcome of the algorithmic decision-making system.
%

Our analysis from an interventions point of view of counterfactual explanations (CFEs) enables us to show three theoretical results: i) CFE-based actions do not guarantee recourse; ii) when they do, they are often sub-optimal in terms of cost; and iii) recourse may be achieved at minimal cost via structural counterfactuals~\cite{pearl2013structural} given the underlying causal model capturing the true dependencies between variables. 
%

% While we believe these results constitute an important step forward in the field, unfortunately our \emph{recourse via minimal intervention} approach also suffers from practical limitations (refer to Section~\ref{sec:050discussion}), as it requires knowledge of the true causal model which is rarely available. We remark though that recourse approaches based on counterfactual explanations were already making implicit unrealistic assumptions about the underlying causal world. Thus, we expect that our work will have a significant impact in the community and trigger  follow-up work addressing the current shortcomings (e.g., alternative world models, and more real-world experiments).

While we have remarked that our proposed approach suffers from practical limitations (requirement for knowledge of the true causal model; see Section~\ref{sec:050discussion}), it is important to consider the context of algorithmic recourse literature where existing approaches based on counterfactual explanations already making implicit unrealistic assumptions about the underlying causal world (i.e., that of independence). In this work, we have demonstrated (both theoretically and empirically) why our proposed formulation for \emph{recourse via minimal intervention} seems the right approach to solve the recourse problem in general real-world settings, where  individuals are affected by algorithmic decision-making systems. 

In summary, we believe that our work is novel and of sufficient conceptual importance for the NeurIPS community, and we expect that it will trigger significant follow-up work addressing the current shortcomings.


% \hl{Resubmission Text:}
% An earlier version of our submission was submitted to ICML 2020.

% We received unanimously positive comments from the reviewers and meta-reviewer on the work's novelty, formalism, and pedagogical value in its introduction and discussion (parts of which have been amended and are now in the supplementary material). Our meta-reviewer commented that ``The proposed formulation is quite novel and the way it is motivated and discussed is also very illuminating.''

% Despite receiving 3 weak accepts (out of 3 reviews), the paper was rejected based on the following main concerns (quoted from the ICML meta-review):
% 1) There is not much empirical work, nor are there any rigorous proofs; and 
% 2) The baselines used in this work are not a great representation of the state of the art.

% In the new version of the paper, we have addressed the concerns by
% (i) presenting our main theoretical results in the form of two propositions and one corollary, which are formally proven in the Appendix;
% (ii) clarifying that up to the best our knowledge no previous work has formally studied the translation from counterfactual explanations to recourse actions. 



% \hl{Confidential comment to PC:} This is a resubmission from an ICML rejected paper, which triggered further work with an additional collaborator that focuses on solving some the practical limitations discussed in the current submission, see NeurIPS submission \#5268. Unfortunately, due to the (somewhat surprising) ICML rejection, both pieces of work now ended up being submitted to NeurIPS 2020. We would like to remark that, while submission \#5268 builds on the present submission, we believe that both papers constitute a significant contribution in their own right, and thus we decided not to merge them into a single article (this would also have been difficult to do, given the time constraints caused by the ICML decision postponement). Nevertheless, if the program committee were of the opinion that the papers should be merged, we would be willing to do so.
% %\bernhard{could add: If the program committee were of the opinion that the papers should be merged, we would be willing to do so.}



==> _bu_050realistic.tex <==
\hl{here}

Additionally, \eqref{eqn:nearest-cf-causal} also enables a new class of feasibility constraints, $\mathcal{F}$. Whereas prior work distinguished only between actionable (or mutable) and non-actionable (or immutable) variables~\cite{ustun2019actionable}, the incorporation of causal structure allows for a finer separation of these terms. Specifically, we can distinguish between i) immutable (e.g., sex); ii) actionable (e.g., bank balance); and iii) mutable but non-actionable (e.g., credit-score) variables. Intuitively, the latter variable type is not directly actionable by the individual, but may change as a consequence of a change to its causal ancestors (e.g., regular debt payment).\footnote{Of course, this example assumes that a bank would not recommend fraudulent actions that may allow direct intervention on credit-score.}
%
In the following section, we provide further real-world examples on selecting the \emph{form}, \emph{feasibility}, and \emph{scope} of interventions, which may be amended to and jointly solved in \eqref{eqn:nearest-cf-causal}.
% to review Appendix~\ref{app:realistic}


% Having specified the context- and individual-dependent intervention form and feasibility constraints~\cite{barocas2020hidden}, the optimization problem in \eqref{eqn:general_assignment_formulation_hard} may be solved by building on existing frameworks for generating nearest counterfactual explanations, including gradient-based, evolutionary-based, heuristics-based, or verification-based approaches as referenced in Section \ref{sec:020background}.
% %
% While out of scope of the current work, for the demonstrative examples below, we extended the open-source code of MACE~\cite{karimi2020model}; we will submit a pull-request to the respective repository.

\hl{here}

Additionally, while our discussion has thus far focused on \emph{structural (a.k.a. hard)} interventions~\cite{pearl2000causality} where graph edges incident on the acted upon variable are severed,
%
an analogous closed-form assignment can be written for \emph{additive (a.k.a. soft)} interventions~\cite{eberhardt2007interventions}: 
%
\begin{equation}
  \begin{aligned} % \nonumber
    \xSCFScalar_i = [i \in I] \cdot \deltaScalar_i + \big( \xFScalar_i + f_i(\pascf_i) - f_i(\paf_i) \big) \\
  \end{aligned}.
  \label{eqn:general_assignment_formulation_soft}
\end{equation}

\noindent where ancestral changes continue to propagate to the intervened variable, even in presence of an additive intervention.
%
Building support for both forms of interventions above is necessary for modelling realistic recourse settings.
%
For instance, we may allow for additive interventions on savings in \textbf{Example~1} so the effect of changes in income would continue to accumulate in savings. Alternatively, we may perform a structural intervention on temperature in \textbf{Example~2}, e.g., by creating a climate controlled green-house, to prevent the natural effect of altitude change on temperature.
%
In the following section, we provide further real-world examples on selecting the \emph{form}, \emph{feasibility}, and \emph{scope} of interventions, which may be amended to and jointly solved in \eqref{eqn:nearest-cf-causal}.

\hl{here}

==> commands_bu.tex <==
\usepackage{lipsum}
\usepackage{color, soul}

\usepackage{enumerate}
\usepackage{bbm}
\usepackage{amsmath}
% \usepackage{unicode-math} % remove, as it throws errors in overleaf
\usepackage{amsmath,amsthm,amssymb}
\usepackage{mathtools}
% \usepackage[algoruled,vlined,nofillcomment]{algorithm2e}
\usepackage{listings}
\usepackage{multirow}
\usepackage{hhline}
\usepackage{changepage} % used for adjustwidth (for large tables)
\usepackage{adjustbox}
\usepackage{subcaption} % subfigure is obsolete and doesn't work with listings; using subcaption instead
\usepackage{tikz}


\usepackage{booktabs}
\usepackage{siunitx}
% \usepackage{unicode-math} % does not work with pdflatex
% \setmathfont{xits-Math}
\newcommand*{\noPrior}{\ensuremath{\mdlgwhtcircle}}
\newcommand*{\quarterPrior}{\ensuremath{\circleurquadblack}}
\newcommand*{\halfPrior}{\ensuremath{\circlerighthalfblack}}
\newcommand*{\threeQuarterPrior}{\ensuremath{\blackcircleulquadwhite}}
\newcommand*{\fullPrior}{\ensuremath{\mdlgblkcircle}}

\newcommand{\zshade}{\cellcolor{gray!25}}
\newcommand{\zpm}[2]{#1\,{\tiny$\pm$\,#2}}
\newcommand{\SAT}{\mathsf{SAT}}
\newcommand{\indep}{\perp \!\!\! \perp}
\newcommand{\argmin}{\mathop{argmin}}
\newcommand{\argmax}{\mathop{argmax}}


% \usepackage{colortbl} % https://stackoverflow.com/a/57222641
% \usepackage[table]{xcolor} % https://tex.stackexchange.com/a/5365
% \PassOptionsToPackage{table}{xcolor, }



\newcommand{\bernhard}[1]{\textbf{\color{orange}~BS:}{~\color{blue}#1}}






\newcommand{\zmat}[1]{\MakeUppercase{\boldsymbol{#1}}}
\newcommand{\zvec}[1]{\boldsymbol{#1}} % for normal variables
\newcommand{\zset}[1]{\mathbb{#1}}
\newcommand{\zrv}[1]{\mathrm{#1}} % for random variables (assume no vectors)

\newcommand{\htheta}{h}

% \newcommand{\factual}{\mathbf{x}^{F}}
% \newcommand{\flabel}{\mathbf{y}^{F}}
% \newcommand{\scf}{\mathbf{x}^{SCF}}
% \newcommand{\cflabel}{\mathbf{y}^{SCF}}
% \newcommand{\params}{\theta}
% \newcommand{\fdo}{\text{\Lightning} \mathbf{z}}
% \newcommand{\fdelta}{\Delta \mathbf{z}}
% \newcommand{\latent}{\mathbf{z}}


\newcommand{\variable}[1]{\texttt{#1}}

\newcommand{\yF}{y^\texttt{F}}
\newcommand{\ySCF}{y^\texttt{SCF}}
\newcommand{\xF}{\zvec{x}^\texttt{F}}
\newcommand{\xFScalar}{x^\texttt{F}}
\newcommand{\xSCFScalar}{x^\texttt{SCF}}
\newcommand{\xCFE}{\zvec{x}^\texttt{CFE}}
\newcommand{\xCFEnearest}{\zvec{x}^\texttt{*CFE}}
\newcommand{\xSCF}{\zvec{x}^\texttt{SCF}}
\newcommand{\xSCFnearest}{\zvec{x}^\texttt{*SCF}}
\newcommand{\xAny}{\zvec{x}}
\newcommand{\xAnyScalar}{x}

\newcommand{\doop}{\mathrm{do}}
\newcommand{\pa}{\zvec{\mathrm{pa}}}
\newcommand{\paf}{\zvec{\mathrm{pa}}^\texttt{F}}
\newcommand{\pascf}{\zvec{\mathrm{pa}}^\texttt{SCF}}

\newcommand{\scmModel}{\mathcal{M}}
\newcommand{\scmGraph}{\mathcal{G}}
\newcommand{\ffinverse}[1]{\zset{F}(\zset{F}^{-1}({#1}))}
\newcommand{\fafinverse}[1]{\zset{F}_{\actionSet}(\zset{F}^{-1}({#1}))}
\newcommand{\fastarfinverse}[1]{\zset{F}_{\actionSetStar}(\zset{F}^{-1}({#1}))}

\newcommand{\deltaVector}{\zvec{\delta}}
\newcommand{\deltaVectorStar}{\zvec{\delta}^*}
\newcommand{\deltaScalar}{\delta}
\newcommand{\deltaScalarStar}{\delta^*}

\newcommand{\actionScalar}{a}
\newcommand{\actionSet}{\mathbb{A}}
\newcommand{\actionSetStar}{\mathbb{A}^*}




\newcommand{\amir}[1]{{\color{blue} Amir: (#1)}}
\newcommand{\bernhard}[1]{\textcolor{orange}{\textbf{Bernhard:} #1}}
\newcommand{\TBC}[1]{\textcolor{red}{\textbf{TBC}: #1}}
\newcommand{\iv}[2][]{{\color{blue} (IV: #2)}}

\newcommand{\distance}{$\delta^*$}
\newcommand{\coverage}{$\Omega^*$}
\newcommand{\realtime}{$\tau^*$}
\newcommand{\divrsity}{$\psi$}
\newcommand{\sparsity}{$\zeta$}


\usepackage{thmtools, thm-restate}

% math environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]


\usepackage{tikz}
% Tikz settings optimized for causal graphs.
% Just copy-paste this part
\usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning}
\tikzset{
    -Latex, auto, node distance = 0.5 cm and 0.5 cm, semithick,
    state/.style = {circle, draw, minimum width = 0.7 cm},
    inter/.style = {rectangle, draw, minimum width = 0.7 cm, minimum height = 0.7 cm},
    point/.style = {circle, draw, inner sep = 0.04cm, fill, node contents = {}},
    bidirected/.style = {Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}

% << For circles in table >>
% https://tex.stackexchange.com/a/488962
% \newcommand*\emptycirc[1][1ex]{\tikz\draw[thick] (0,0) circle (#1);} 
% \newcommand*\halfcirc[1][1ex]{%
%   \begin{tikzpicture}
%   \draw[fill] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
%   \draw[thick] (0,0) circle (#1);
%   \end{tikzpicture}}
% \newcommand*\fullcirc[1][1ex]{\tikz\fill (0,0) circle (#1);}

\newcommand*\emptycirc[1][.9ex]{\tikz\draw (0,0) circle (#1);} 
\newcommand*\halfcirc[1][.9ex]{%
  \begin{tikzpicture}
  \draw[fill] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
  \draw (0,0) circle (#1);
  \end{tikzpicture}}
\newcommand*\fullcirc[1][.9ex]{\tikz\fill (0,0) circle (#1);}
% \newcommand*\fullcirc[1][.9ex]{\tikz\fill [fill=gray!25] (0,0) circle (#1);}


\newcommand{\yy}{\fullcirc} % {\checkmark}
\newcommand{\pp}{\halfcirc} % {$\sim$}
\newcommand{\xx}{\emptycirc} % {x}
\newcommand{\qq}{?}
\newcommand{\ee}{$\mathcal{E}$}
\newcommand{\rr}{$\mathcal{R}$}
\newcommand{\citeartelt}{\citep{artelt2019efficient, artelt2019computation, artelt2020convex}}

